Two-Stream CNN with Loose Pair Training for Multi-modal AMD Categorization

This paper studies automated categorization of age-related macular degeneration (AMD) given a multi-modal input, which consists of a color fundus image and an optical coherence tomography (OCT) image from a specific eye. Previous work uses a traditional method, comprised of feature extraction and classifier training that cannot be optimized jointly. By contrast, we propose a two-stream convolutional neural network (CNN) that is end-to-end. The CNN's fusion layer is tailored to the need of fusing information from the fundus and OCT streams. For generating more multi-modal training instances, we introduce Loose Pair training, where a fundus image and an OCT image are paired based on class labels rather than eyes. Moreover, for a visual interpretation of how the individual modalities make contributions, we extend the class activation mapping technique to the multi-modal scenario. Experiments on a real-world dataset collected from an outpatient clinic justify the viability of our proposal for multi-modal AMD categorization.

==> instance_tab.tex <==
\begin{table*} [tb!]
%    \renewcommand{\arraystretch}{1.2}
    \caption{\textbf{Class activation map images for visualization}. Each column is from one example. The first row is slit-lamp image, while the second row is its class activation map image. The third row is the resized nuclear region, while the next row is its class activation map image. Red color indicates strong evidence of prediction while blue color indicates less impact.}
    \label{tab:heat-map}
    \centering
    \scalebox{0.95}{
        \begin{tabular}{@{} c*{5}c @{}}
\toprule
%\hline
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/SquareCrop_ImageData_224x224/DRIVE001_IMAGES_IM000360} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/SquareCrop_ImageData_224x224/DRIVE001_IMAGES_IM000457} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/SquareCrop_ImageData_224x224/DRIVE001_IMAGES_IM000335} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/SquareCrop_ImageData_224x224/DRIVE001_IMAGES_IM000712} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/SquareCrop_ImageData_224x224/DRIVE001_IMAGES_IM000454} &
             \\
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/slit_lamp_fusionImgs/DRIVE001_IMAGES_IM000360} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/slit_lamp_fusionImgs/DRIVE001_IMAGES_IM000457} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/slit_lamp_fusionImgs/DRIVE001_IMAGES_IM000335} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/slit_lamp_fusionImgs/DRIVE001_IMAGES_IM000712} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/slit_lamp_fusionImgs/DRIVE001_IMAGES_IM000454} &
             \\
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/PredCrop_ImageData_Resize224x224/DRIVE001_IMAGES_IM000360} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/PredCrop_ImageData_Resize224x224/DRIVE001_IMAGES_IM000457} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/PredCrop_ImageData_Resize224x224/DRIVE001_IMAGES_IM000335} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/PredCrop_ImageData_Resize224x224/DRIVE001_IMAGES_IM000712} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/PredCrop_ImageData_Resize224x224/DRIVE001_IMAGES_IM000454} &
             \\
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/nuclear_fusionImgs/DRIVE001_IMAGES_IM000360} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/nuclear_fusionImgs/DRIVE001_IMAGES_IM000457} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/nuclear_fusionImgs/DRIVE001_IMAGES_IM000335} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/nuclear_fusionImgs/DRIVE001_IMAGES_IM000712} &
             \includegraphics[width=2.15cm,height=2.15cm]{pictures/nuclear_fusionImgs/DRIVE001_IMAGES_IM000454} &
            \\
            {\scriptsize Ground truth=1.3} & {\scriptsize Ground truth=2.0} & {\scriptsize Ground truth=3.0} & {\scriptsize Ground truth=4.0} & {\scriptsize Ground truth=5.0} \\
            {\scriptsize P(Slit-lamp)=2.1} & {\scriptsize P(Slit-lamp)=2.5} & {\scriptsize P(Slit-lamp)=3.1} & {\scriptsize P(Slit-lamp)=4.0} & {\scriptsize P(Slit-lamp)=4.4} \\
            {\scriptsize P(Nuclear)=1.3} & {\scriptsize P(Nuclear)=2.1} & {\scriptsize P(Nuclear)=3.2} & {\scriptsize P(Nuclear)=3.8} & {\scriptsize P(Nuclear)=4.5} \\ 

\bottomrule
\end{tabular}
}
\end{table*}

